Box-Adapt: Domain-Adaptive Medical Image Segmentation using Bounding BoxSupervision

Deep learning has achieved remarkable success in medicalimage segmentation, but it usually requires a large numberof images labeled with fine-grained segmentation masks, andthe annotation of these masks can be very expensive andtime-consuming. Therefore, recent methods try to use un-supervised domain adaptation (UDA) methods to borrow in-formation from labeled data from other datasets (source do-mains) to a new dataset (target domain). However, due tothe absence of labels in the target domain, the performance ofUDA methods is much worse than that of the fully supervisedmethod. In this paper, we propose a weakly supervised do-main adaptation setting, in which we can partially label newdatasets with bounding boxes, which are easier and cheaperto obtain than segmentation masks. Accordingly, we proposea new weakly-supervised domain adaptation method calledBox-Adapt, which fully explores the fine-grained segmenta-tion mask in the source domain and the weak bounding boxin the target domain. Our Box-Adapt is a two-stage methodthat first performs joint training on the source and target do-mains, and then conducts self-training with the pseudo-labelsof the target domain. We demonstrate the effectiveness of ourmethod in the liver segmentation task. Weakly supervised do-main adaptation

==> abstract_v1.tex <==
\begin{abstract}
Accurate segmentation is one of the essential tasks when working with medical images. 
Recently, deep convolutional neural networks achieved state-of-the-art performance in many segmentation benchmarks. 
Regardless of the network architecture, the deep learning-based segmentation methods view the segmentation problem as a supervised task that requires a relatively large number of annotated images.  Acquiring a large number of annotated medical images is time-consuming, and high-quality segmented images (i.e., strong labels) by human experts are expensive to collect.
In this paper, we propose a method that achieves competitive accuracy from a ``weakly annotated'' image where the weak annotation is obtained via a 3D bounding box denoting an object of interest. Our method, called ``3D-BoxSup'', employs a positive-unlabeled learning framework to learn segmentation masks from 3D bounding boxes. Specially,   we consider the pixels outside of the bounding box as positively-labeled data and the pixels inside the bounding box as unlabeled data. Our method can suppress the negative effects of pixels residing between the true segmentation mask and the 3D bounding box and produce accurate segmentation masks. We apply our method to segment brain tumor. The experimental results on the BraTS 2017 dataset.

\keywords{First keyword  \and Second keyword \and Another keyword.}
\end{abstract}
